Influence of crystal structure on charge carrier effective masses in BiFeO$_3$

Ferroelectric-based photovoltaics have shown great promise as a source of renewable energy, thanks to their in-built charge separation capability, yet their efficiency is often limited by low charge carrier mobilities. In this work, we compare the photovoltaic prospects of various phases of the multiferroic material BiFeO$_3$ by evaluating their charge carrier effective masses using first-principles simulations. We identify a tetragonal phase with the promising combination of a large spontaneous polarisation and relatively light charge carriers. From a systematic study of the octahedral distortions present in BiFeO$_3$, we explain the relationship between structure and effective masses in terms of the changes to the orbital character and overlap at the band edges that result from changes in the geometry. The findings in this study provide some design principles to engineer desired effective masses in BiFeO$_3$ and similar materials through manipulation of their crystal structures in experimentally accessible ways.

==> __latexindent_temp.tex <==
plays an important role in the BPVE in BFO [114]. According to this model, charge carrier separation in the BPVE is driven by coherent excitations, rather than a built-in electric field. In a monodomain FE material, therefore, the magnitude and direction of the photocurrent does not necessarily depend on the magnitude or orientation of the FE polarisation; it is sufficient to have an absence of inversion symmetry. Extrinsic mechanisms include factors such as FE domains, point defects and band bending due to surfaces.
